Consistency and Variation in Kernel Neural Ranking Model

This paper studies the consistency of the kernel-based neural ranking model K-NRM, a recent state-of-the-art neural IR model, which is important for reproducible research and deployment in the industry. We find that K-NRM has low variance on relevance-based metrics across experimental trials. In spite of this low variance in overall performance, different trials produce different document rankings for individual queries. The main source of variance in our experiments was found to be different latent matching patterns captured by K-NRM. In the IR-customized word embeddings learned by K-NRM, the query-document word pairs follow two different matching patterns that are equally effective, but align word pairs differently in the embedding space. The different latent matching patterns enable a simple yet effective approach to construct ensemble rankers, which improve K-NRM's effectiveness and generalization abilities.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> tables/tab_ensemble_stats.tex <==
\begin{table*}
\centering
\caption{Statistics of 10 Ensemble Pattern-A\&B runs. 
\label{table:stats-ensemble} 
\zhuyun{the variance is not right}
}
\begin{tabular}{@{}l|l|l|l||l|l|l||l@{}}
\hline
 & \multicolumn{3}{c||}{\textbf{Testing-SAME}} & \multicolumn{3}{c||}{\textbf{Testing-DIFF}} & \textbf{Testing-RAW} \\ \hline
\multicolumn{1}{c|}{\textbf{Statistic}} & \multicolumn{1}{c|}{\textbf{NDCG@1}} & \multicolumn{1}{c|}{\textbf{NDCG@3}} & \multicolumn{1}{c||}{\textbf{NDCG@10}} & \multicolumn{1}{c|}{\textbf{NDCG@1}} & \multicolumn{1}{c|}{\textbf{NDCG@3}} & \multicolumn{1}{c||}{\textbf{NDCG@10}} & \multicolumn{1}{c}{\textbf{MRR}} \\ \hline
Minimum & 0.3238 & 0.3735 & 0.4601 & 0.3858 & 0.3791 & 0.4657 & 0.3976 \\ 
Mean & 0.3303 & 0.3826 & 0.4669 & 0.3950 & 0.3866 & 0.4699 & 0.4045 \\ 
Maximum & 0.3469 & 0.3908 & 0.4736 & 0.4005 & 0.3942 & 0.4725 & 0.4086 \\ 
Standard Deviation & 0.0068 & 0.0046 & 0.0044 & 0.0051 & 0.0047 & 0.0022 & 0.0035 \\ \hline
\end{tabular}
\end{table*}

==> v1/conclusion.tex <==
\section{Conclusion}
Stability and reproducibility are two very important aspects for any machine learning model. Deep learning models have been found to have high variance due to the use of certain optimization algorithms and use of stochastic gradient methods. In this paper, we explore the instabilities in K-NRM, a state of the art deep learning model for the task of adhoc retrieval. Our experiments indicated a high variance in the results and we further studied the sources of variance in the model. 

We showed that there were mainly two patterns of learning to rank weights which indicated the initialization of the model parameters was the cause of variance in the model. We further studied the query document similarities which indicated that the model had clustering properties where each kernel bin represents certain properties of the concerned query document words such as synonyms.  To further improve the model performance and make it more stable, we use an ensemble of the base models leading to a  higher performance with an increase of 16\% over the base models. We observe that there exists variance both within the same pattern and across patterns caused due to the random initializations. This leads to a improvement in the performance for all ensemble models. We also further show that the ensemble models have lower variance making the model more generalizable. 

==> v1/introduction.tex <==
\section{Introduction}

%Recent success of deep learning in natural language processing (NLP) tasks such as question answering, conversational agents, paraphrasing and summarization has fueled interest in neural models for IR. The basic architecture for an IR neural model consists of generating a representation for the query and the document followed by a relevance matching model. Several models \cite{huang2013learning,shen2014latent}have been proposed based on this approach for neural-IR. However, these proposed approaches are based on existing NLP tasks and as pointed out by Guo et al. \cite{guo2016deep}, the problem of ad-hoc retrieval differs from other NLP tasks. Unlike other NLP tasks where the focus is on semantic matching with the need to understand the meaning of the inputs, ad-hoc retrieval is mainly based on relevance matching between the query and the document, the query usually being short and not descriptive. Targeting these discrepancies, Guo et al.\citep{guo2016deep} propose a deep relevance matching algorithm which uses a histogram mapping approach to model the different similarity levels of term frequency matches between the document and query terms. However, this model is not trainable end-to-end due to a non-differentiable mapping function. Xiong et al. \cite{xiong2017end} further propose a kernel pooling approach which is end-to-end trainable and similarly models different levels of similarity through soft term frequency matches. 

Recently deep learning models in information retrieval have started to show success over traditional techniques. One recent success in neural-IR is the Kernel-based Neural Ranking Model (\texttt{KNRM})~\citep{xiong2017end} which 
models word-word soft matches using word embeddings and use a new kernel pooling technique to learn matching patterns. The high capacity of neural models enables \texttt{K-NRM} to encode rich information from user feedbacks in the word embeddings and to learn soft match patterns tailored for matching queries and documents.
However,  the high capacity of the model, as well as the non-convexity of the optimization problem, may lead to high variance. The effectiveness of the model may be affected by the randomness in the training procedure. This paper asks the following research questions:

1. How much variance is there across multiple stochastically trained \texttt{K-NRM} models?

2.If there is variance, how do the models differ in the learned soft-matching patterns? 

3. Can we leverage the model differences to improve effectiveness and stability?

To answer the first question, We  study the stability of \texttt{K-NRM} by comparing the effectiveness of repeated runs of the models. Experimental results show that the overall effectiveness is stable across runs. However, when comparing the  at individual query level, we found that the document rankings for a query differs a lot in the multiple \texttt{K-NRM} runs. 

Next, to interpret the model differences, we analyze the query-document word pair similarities in different runs of the model. This analysis shows that each run has its own ways of grouping query-document word pairs, forming distinct matching patterns. 

Finally, we leverage the model differences to explore the ensemble of multiple independent runs.  Since the document rankings for a query varies across runs, the ensemble model can pull up the best documents which is agreed by the majority runs. Experimental results show that the ensemble model boosts the performance, prevents over-fitting, and reduces the variance. The experiment also shows that ensembles covering different latent matching patterns outperformed ensembles with only a single pattern, demonstrating that each latent pattern has its distinctive learning properties and is beneficial to combine them. 



%Haber et al. \cite{haber2017stable} discuss the well known difficulties in training deep learning models, and identify the causes for lack of stability and high variance as the dimensionality and non-convexity of the optimization problem. 
%Generally, stochastic gradient methods have been used and the performance of the model is highly dependent on the choice of optimization algorithm and the sample size. \cite{byrd2012sample,bottou2016optimization}. As discussed in Ju et al.\cite{ju2017relative}, a technique proven to reduce variance and improve performance in deep learning models is to average over multiple stochastically trained networks. 

%In this paper, we identify that stability and reproducibility are important aspects to be addressed for a deep learning model. We employ the K-NRM model\cite{xiong2017end} and show with repeated experiments that the model lacks stability due to different parameter initializations. We show that by using an ensemble of the base models of K-NRM, we can reduce the variance in the model and boost performance. We further analyze the interpretability of the model by providing qualitative analysis on the differences in the query-document word pair similarities over the different runs of the model.

==> v1/k-nrm.tex <==
\section{Overview of K-NRM} \label{section:knrm}
\texttt{K-NRM} takes as input a query $q$ and a
document $d$.  Each word $t$ is represented by an embedding vector $v_t$.
A translation matrix $M$ is formed in which each element is the cosine similarity between the embeddings of a query word and a document word.  


%\cx{Merge this section into related work?}
%\texttt{K-NRM} \cite{xiong2017end} takes as input a query $q$ and a
%document $d$, and outputs a relevance score $f(d,q)$ indicating
%the relevance between q and d.

%a kernel pooling approach using Gaussian kernels instead of histogram mappings which helps in learning the word embeddings. This apporach makes the model end to end trainable. 

%Each word $t$ is represented by an embedding vector $v_t$. Then it constructs a translation matrix $M$ where each element is the cosine similarity between the embeddings of a query word and a document word.  

\begin{align*}
t &\implies v_t \tag{Word Embedding} \\
M_{ij} &= \cos (v_{t_i^q}, v_{t_j^d}) \tag{Translation Matrix} \\
\end{align*}

Gaussian kernels with different mean values ranging from $[-1, 1]$ are used to assign the query document word pairs to the corresponding similarity bins which also range from $[-1, 1]$. 
\begin{align*}
K_k(M_i) &= \sum_j \exp \Bigg( - \frac{(M_{ij} - \mu_k)^2}{2\sigma_k^2} \Bigg) \tag{Gaussian Kernel} \\
K(M_i) &= \{K_1(M_i), \dots, K_K(M_i)\} \tag{Kernel Pooling} \\
\end{align*}

The kernels `count' the soft-matches at different similarity levels. A kernel with $\mu=1$ corresponds to an exact-match term frequency feature. A kernel with $\mu=0.5$ corresponds to the frequency of query-document word pairs that have a similarity score near $0.5$.  The logarithmic feature values in these bins are summed over different query terms, producing $K$ features for the query-document pair, each corresponding to the soft-term frequency (soft-TF) in one kernel.

\begin{align*}
\phi(M) &= \{\sum^{n}_{i=1} \log K_1(M_i),...,\sum^{n}_{i=1} \log K_K(M_i)\}\tag{Soft-TF features}  \\
\end{align*}
Finally, a learning-to-rank layer is used which combines these kernel features into the final ranking score. 
\begin{align*}
f(q, d) &= \tanh (w^T \phi(M) + b) \tag{Learning to Rank}\\
\end{align*}

The whole model is stochastically trained on click log data. The model jointly optimizes word embedding and learning-to-rank weights via end-to-end learning. However, the training of \texttt{K-NRM} may cause instability due to the randomness in the training procedure and the non-convexity of the optimization problem. This issue is studied in the rest of paper. We first  describes experimental setups in Section 4. Section 5 explored the variance of multiple independent \texttt{K-NRM} runs; Section 6 investigate divergence in the matching patterns learned by the multiple runs; Section 8 studied the effectiveness of combining diverged runs using ensemble models. We conclude in Section 8.

%\zhuyun{Add methodology/research question}

==> v1/word_pair_analysis_old.tex <==

% \end{table*}


\section{Latent Matching Patterns} \label{subsection:variance}
In this section, we analyze the representations of the kernel bins and the patterns in the learning-to-rank weights generated from multiple runs of K-NRM model to determine the sources of variance. We study the notion of query-document word pair similarities and learning-to-rank weights with respect to the ad-hoc information retrieval task. 

We observe that all  the learning-to-rank weights generated from the 50 runs follow 2 patterns \zhuyun{all runs or most runs?}. We randomly pick 5 of those runs and show the show the learning-to-rank weights generated in Figure \ref{fig:ltr_weights}. 


\begin{figure}[h]
\centering
 \includegraphics[width=\linewidth]{figures/ltr-weights-scatter.png}
  \caption{Learning-To-Rank weights in 5 different runs \zhuyun{larger font size for labels and legends}} 
  \label{fig:ltr_weights}
\end{figure}

From the figures, we can observe that Run1 and Run4 have similar weight patterns while Run2, Run3 and Run5 have similar pattern of weights. Depending on the initializations of the word embeddings and learning-to-rank weights, the weights converge at different optima. This can be viewed as a clustering problem, where each kernel bin represents a property of the query-document word pairs. For example, the synonyms being clustered in one bin, segmented words being clustered in another. In this model, the query-document word pair similarity score is not directly proportional to the relevance score. The clustering property of this model can be viewed clearly through the heat maps which capture the query-document word pair movements in different runs. Here, we study the word pair movements for the different runs belonging to the same pattern and further pick a run from one pattern and study its properties with respect to a run from the other pattern to be able to compare and contrast the movements. Figures \ref{fig:heatmaps} show the heat maps generated for Run2 versus the rest of the runs.  

The runs 2,3 and 4 have similar learning-to-rank weights and hence the clustering happens similarly with the same cluster centers. This is seen from the figures \ref{fig:heatmap_run23} and \ref{fig:heatmap_run25} where there is a diagonal relationship between the word pairs in these runs. However, run1 and run2 have different learning-to-rank weights and hence the cluster centers are different and there is word pair movement as seen in Figure \ref{fig:heatmap_run21}. For example, in the the 0.9 bin in Run1, majority of word pairs correspond to segmentation errors such "Man", and "ga" (corresponding to Manga) or "home" and "page" (corresponding to homepage). These word pairs move to bin 0.5 in Run2. We also observe that there is random movement of word pairs to the 0.1 bin in Figure \ref{fig:heatmap_run24} and \ref{fig:heatmap_run25} and this can also be a cause of variance both within and across the runs of same patterns and different patterns. 

The query-documents for heat maps are sampled from training set where 1000 queries are selected randomly and 30 documents are selected from each query. The query-documents from the sampled training set and test set are used for this analysis. The query-document word pairs are assigned to its corresponding nearest kernel bin and 100 query-document word pairs are selected randomly from each kernel bin.


% \begin{figure}[h]
%   \begin{minipage}[b]{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/14.png}
%     \caption{Learning-To-Rank weights for Run1 and Run4}
%     \label{fig:ltr14}
%   \end{minipage}
%   \hspace{1cm}
%   \begin{minipage}[b]{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/235.png}
%     \caption{Learning-To-Rank weights for Run2, Run3 and Run5}
%     \label{fig:ltr235}
%   \end{minipage}
%   \zhuyun{Put all runs in one figure? The current figures do not show the difference between run1/4 and run2/3/5 clearly.}
% \end{figure}


% \begin{table*}
% \centering
% \caption{K-NRM with Fixed-Seed-Embed}
% \label{table:fix-word2vecweights}
% \begin{tabular}{@{}l|lll|lll|l@{}}
% \toprule
% \textbf{} & \textbf{\begin{tabular}[c]{@{}l@{}}DCTR\\ NDCG@1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}DCTR\\ NDCG@3\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}DCTR\\ NDCG@10\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}TACM\\ NDCG@1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}TACM\\ NDCG@3\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}TACM\\ NDCG@10\end{tabular}} & \textbf{MRR} \\ \midrule
% Minimum & 0.2703 & 0.3395 & 0.4287 & 0.3082& 0.3308 & 0.4311 & 0.3433 \\ 
% Mean & 0.2806 & 0.3475 & 0.4380 & 0.3272 & 0.3397 & 0.4390 & 0.3554 \\ 
% Maximum & 0.3027 & 0.3633 & 0.4546 & 0.3384 & 0.3546 & 0.4478 & 0.3734 \\ 
% Variance & 0.000111 & 0.000066 & 0.000056 & 0.000084 & 0.000056 & 0.000029 & 0.000075 \\ \bottomrule
% \end{tabular}
% \end{table*}

\begin{figure*}[h]
\centering
  \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figures/resized_heatmap_run2_run1.png}
    \caption{Run2 to Run1}
    \label{fig:heatmap_run21}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figures/resized_heatmap_run2_run3.png}
    \caption{Run2 to Run3}
    \label{fig:heatmap_run23}
   \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figures/resized_heatmap_run2_run4.png}
    \caption{Run2 to Run4}
    \label{fig:heatmap_run24}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figures/resized_heatmap_run2_run5.png}
    \caption{Run2 to Run5}
    \label{fig:heatmap_run25}
  \end{subfigure}
 \caption{Movement of word pairs from Run2 to different runs }  \zhuyun{labels and legends are still too small to read} \arpita{Now?}
 \label{fig:heatmaps}
\end{figure*}

% From the previous section, we can see that there is a difference in the performance of the model in different runs because of the difference in the weight initializations. 

